A Data-Centric Optimization Framework for Machine Learning

Rapid progress in deep learning is leading to a diverse set of quickly changing models, with a dramatically growing demand for compute. However, as frameworks specialize performance optimization to patterns in popular networks, they implicitly constrain novel and diverse models that drive progress in research. We empower deep learning researchers by defining a flexible and user-customizable pipeline for optimizing training of arbitrary deep neural networks, based on data movement minimization. The pipeline begins with standard networks in PyTorch or ONNX and transforms computation through progressive lowering. We define four levels of general-purpose transformations, from local intra-operator optimizations to global data movement reduction. These operate on a data-centric graph intermediate representation that expresses computation and data movement at all levels of abstraction, including expanding basic operators such as convolutions to their underlying computations. Central to the design is the interactive and introspectable nature of the pipeline. Every part is extensible through a Python API, and can be tuned interactively using a GUI. We demonstrate competitive performance or speedups on ten different networks, with interactive optimizations discovering new opportunities in EfficientNet.

==> 04_5_case_studies.tex <==
We walk through the optimization process on representative DNN operators, applying the recipe described in Section~\ref{sec:recipe}. 

\subsection{Mish Activation}
\begin{figure}
    \centering
    \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=0.4\linewidth]{figures/mish_fwd.pdf}
    \quad
    \includegraphics[width=0.45\linewidth]{figures/mish_bwd.pdf}
    \caption{Before Optimization (intermediate memory: 134.75MiB)}
    \label{fig:mish:before}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=0.425\linewidth]{figures/mish_fwd_after.pdf}
    \quad
    \includegraphics[width=0.425\linewidth]{figures/mish_bwd_after.pdf}
    \caption{After Optimization (intermediate memory: 0MiB)}
    \label{fig:mish:after}
    \end{subfigure}
    \caption{Mish operator SDFG forward pass (left) and the resulting backpropagated graph (right). Colored access nodes correspond to matching data.}
\end{figure}
YOLOv4~\cite{yolov4} is a widely-used network for object detection.
Among other features, it relies on the Mish~\cite{mish} activation: $\mathrm{mish}(x) = x\tanh(\mathrm{softplus}(x))$. As with many operators, Mish is not natively supported by PyTorch, ONNX, nor ONNX Runtime. 

The unoptimized graphs shown in Figure~\ref{fig:mish:before} are simply sequential elementwise applications of the individual primitives used in the activation function (i.e. $\exp$, $\tanh$, $\log$, $+$, $*$). This is typical for a DaCeML kernel since most  are authored using the NumPy/Python frontend and not manually optimized. Notice the bold outline on the intermediate arrays---they are global, and are thus all retained for the backward pass, identical to how operator-graph AD engines would differentiate such a graph.

Applying the generic transformation recipe yields the optimized SDFGs shown in Figure~\ref{fig:mish:after}. Note that the kernels are maximally fused, and the absence of global data-movement stashing intermediate values for differentiation. DaCeML achieves this by applying subgraph fusion prior to differentiation, and then differentiating the fused and scheduled kernel, a capability which all other frameworks lack. 

\subsection{Statistical Normalization}
Statistical normalization operations (e.g., Batch Normalization, Layer Normalization, Group Normalization) are commonplace in modern DNNs. We examine layer normalization~\cite{layernorm}, a primitive widely used in transformer models.
Despite the fact that all normalization operations are similar, their performance varies. All the aforementioned operations perform the general computation $\gamma\cdot\frac{x-\mathbb{E}[x]}{\sqrt{\text{Var}(x) + \epsilon}}+\beta$, but on different dimensions or subsets thereof. 

We find, for example, that PyTorch has two separate implementations for layer and batch normalization.
The implementation of batch normalization can use cuDNN, while layer normalization uses a manually-optimized function. Thus, despite batch normalization being more expensive than layer normalization (due to saving running mean/variance statistics to memory), the former is faster than the latter.

Conversely, DaCeML begins with naive, numpy-like implementations of these operators and uses the same, generic transformation recipe from Section~\ref{sec:pipeline} to produce optimized kernels for these operators.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
\begin{minted}[fontsize=\scriptsize]{python}
@op_implementation(op="Softmax",
                   name="native")
class NativeSoftmax(ONNXForward):
  @staticmethod
  def forward(node, state, sdfg):
    # Get properties and shapes
    axis = node.axis
    reduced_shape = list(copy.deepcopy(
      in_desc_with_name(node, state, 
        sdfg, "input").shape))
    reduced_shape[axis] = 1

    # Operator implementation in numpy
    def prog(input, output):
      max = np.max(input,
        axis=axis).reshape(reduced_shape)
      exp_arr = np.exp(input - max)
      sum = np.sum(exp_arr,
        axis=axis).reshape(reduced_shape)
      output[:] = exp_arr / sum

    return program_for_node(prog, sdfg,
                            state, node)
\end{minted}
    \caption{NumPy Implementation}
    \end{subfigure}\qquad
    \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \includegraphics[height=2.5in]{figures/smax/01_input.pdf}
    \caption{Resulting SDFG}
    \end{subfigure}
    \caption{Softmax implementation in DaCeML.}
    \label{fig:smax}
\end{figure}
\textbf{Softmax}\; The initial naive NumPy implementation of the softmax operator (see Figure~\ref{fig:smax}) %
lowers the ONNX library node to four separate operations: two reductions (computing the maximum value to subtract; and summarizing the contributions for the denominator), and two elementwise operations (exponentiation, division).
In the current mode, three extraneous tensors sized as the input would be generated. We can thus apply the second step of our recipe and locally reduce this data movement.

Fusion of those operators is not trivial, as the dimensions of the maps and reductions differ. The \texttt{greedy\_fuse} method in DaCe automatically expands reductions (via \texttt{ReduceExpansion}) and finds common dimensions to extract out of the maps in the subgraph, which in turn allows to fuse them all to one map. This stores all memory locally, within the map. The end result is shown on Figure~\ref{fig:softmax_transformations}, on the top-left SDFG.

As the global data movement optimization step does not apply in this case, the recipe proceeds to specialize the code to the GPU. 
The code gradually lowers the representation (expanding the two reductions to nested SDFGs), transforms the map to be executed on a GPU (via \texttt{GPUTransformSDFG}), and calls \texttt{WarpTiling} to partition the work in the internal maps across warps. Note that this automatically generates warp-level reductions, and by default \textit{replicates} all computations that have multiple results dependent on reductions (the latter is configurable). This is shown in the top-right SDFG in Figure~\ref{fig:softmax_transformations}.
Lastly, the SDFG is cleaned up via another pass of transformations --- \texttt{HoistState} to move initialization up, another batch of map fusion, and vectorization (shown in the bottom graph of the figure).

The resulting performance matches the performance of state-of-the-art hand-written implementations, such as the PyTorch built-in softmax implementation.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.3\linewidth]{figures/smax/03_fused.pdf}
    \quad
    \includegraphics[width=0.3\linewidth]{figures/smax/05_warptile.pdf}
    \quad
    \includegraphics[width=0.3\linewidth]{figures/smax/07_final.pdf}
    \caption{Softmax SDFG transformations: after subgraph fusion (left), warp tiling (middle), cleanup and vectorization (right).}
    \label{fig:softmax_transformations}
\end{figure}

\textbf{Layer Normalization}\; The same exact recipe that was applied in Softmax can be applied to the Layer Normalization operator. The generated implementation is evaluated in the following section.



==> background.tex <==
\tal{Write this section}
batchnorm/layernorm, 5d tensors, seeing if two different layouts with elementwise get fused (they do)...

We analyze the performance characteristics and optimizations of Tensorflow/XLA running EfficientNet-B0, and identify performance bottlenecks and missed opportunities for optimization.
We also demonstrate how existing inter-operator subgraph optimizations -- which are commonly used in ML frameworks -- are insufficient in a fast moving field like ML. For example, XLA may optimize \texttt{BatchNorm}, but not \texttt{LayerNorm} (the exact example we use is TBD).

\input{dnncompilers.tex}

Intro to SDFG representations of ONNX graphs (context for transformations section).


(discussion) The situation of memory movement is so dire that several GitHub repositories define "MemoryEfficient" versions of some operators, which in practice apply (tasklet) fusion for backprop.

\subsection{Multi-level IR}
Describe how nodes are lowered in multiple stages. Example:

{ONNX Broadcasted MatMul} $\to$ {ONNX Einsum} $\to$ {DaCe BLAS MatMul} $\to$ {DaCe BMM} $\to$ {CUDA strided BMM call}


\subsection{Case Study: Batch Normalization vs. Layer Normalization}

Statistical normalization operations [cite groupnorm layernorm batchnorm instancenorm...] are commonplace in modern deep neural networks.

Two common examples are LayerNorm and BatchNorm. Both operations do $\gamma\cdot\frac{x-\mathbb{E}[x]}{\sqrt{\text{Var}(x) + \epsilon}}+\beta$, but on different dimensions. 
Batchnorm is even more complex than layernorm since it has running mean/variance metrics. However, it turns out that frameworks view things differently and BN is faster than LN, despite the added storage.
(see Table)
We see that XLA behaves differently from JAX. Upon inspecting the generated assembly, it seems that TF+XLA does detect statistical normalization, as the keyword \texttt{FusedBatchNormV3} appears. All in all, very operator specific and won't easily generalize to tomorrow's statistical normalization.







==> impl.tex <==
\section{Implementation}
\oliver{do this section}.We present the DaCeML system using a guide from high-level framework code, lowered to c++ code that is compiled by general purpose compilers.
PyTorch$\to$ ONNX $\to$ DaCe $\to$ transformations $\to$ codegen.


\subsection{Backpropagation}
\oliver{add figures}
We use a symbolic automatic differentiation engine to derive explicit backpropagation graphs in the same data-centric intermediate representation as our forward pass.
\subsection{Usability and Integration}
We describe how our models integrate with PyTorch and how users can use them. We also mention how the ORT fallback approach aids in bootstrapping kernel development.

\subsection{Performance Optimization Workflow}
\oliver{write about cutout}
We describe how our framework facilitates simple and productive performance engineering through the dace framework and white-box optimization.
